Green Flash: Residual Emissions Enshrouded in Low-mass Balmer-break Galaxies at $z\sim5$

Recent James-Webb Space Telescope (JWST) observations have discovered galaxies that are already passively evolving at $z>4$, $\sim1.5$\,Gyr after the Big Bang. Remarkably, some of these galaxies exhibit strong emission lines such as \ha\ and \oiii\ while showing a strong continuum break at $\sim3650$\,\AA\ i.e., Balmer break, giving us a unique insight into the physical mechanisms responsible for early galaxy quenching. In this study, we investigate the nature of four such galaxies at $z=5.10$--$5.78$ identified in the Abell~2744 field, using JWST/NIRCam and NIRSpec data. Our spectral energy distribution (SED) fitting analysis reveals that these galaxies have been mostly quiescent since $\sim100$\,Myr prior to the observed time. We find a higher dust attenuation in the nebular component than in the continuum in all cases. This suggests the presence of dusty star-forming regions or obscured AGN, which could be a {\it residual} signature of past quenching. For one of the galaxies with sufficient medium-band coverage, we derive the \hb+\oiii\ emission line map, finding that the line-emitting region is located in the center and is more compact ($R_e=0.7$\,kpc) than the stellar component ($R_e=0.9$\,kpc). For this specific galaxy, we discuss a scenario where quenching proceeds in the manner of ``outside-in", a stark contrast to the inside-out quenching commonly seen in massive galaxies at later cosmic times.

==> old_sec43.tex <==

\subsubsection{Quenching driven by outflows}
Outflows powered by stellar feedback (e.g., supernovae, stellar winds) or AGNs can reduce or even expel the interstellar medium (ISM) of a galaxy, leading to quenching. Such outflows can form when intense star formation or AGN activity produces energetic winds that carry gas out of the galaxy’s potential well. In massive galaxies, the gravitational potential is deeper, so large-scale outflows can be suppressed; conversely, in less massive systems, it is easier for outflows to remove significant amounts of gas.

A typical indication of outflows is the presence of broad or offset emission-line components \citep[e.g.,][]{belli_star_2024,de_graaff_efficient_2024}. However, our low-resolution spectra do not reveal clear velocity shifts, making it difficult to claim ongoing outflows for these four galaxies. More sensitive, high-resolution spectroscopy (e.g., from ALMA or JWST/NIRSpec IFU data) is required to confirm or rule out outflow signatures.
This galaxy exhibits a smaller emission-line region compared to its stellar component, suggesting that any outflow-driven gas removal could have occurred at an earlier epoch. Additionally, the younger stellar population appears to be more concentrated in the inner region, whereas older stars inhabit the outskirts. Since the outer regions have a shallower gravitational potential, outflows there would be more effective in expelling gas, potentially explaining the current star-formation ``desert” in that region.

 By measuring molecular gas masses and possible high-velocity wings in CO or \cii\ lines, ALMA can detect outflow signatures more definitively. Such data would help confirm whether gas reservoirs have been depleted via outflows in our sample galaxies.
Deeper and higher-resolution spectroscopy (the medium- or high-resolution spectroscopy obtained by the JWST/NIRSpec) could reveal subtle velocity structures that are currently undetectable with low-resolution spectra.


\subsubsection{Quenching driven by radiative heating}
Radiative heating can arise from several sources, including massive stars in HII regions, supernova shocks, and AGNs. When the interstellar medium (particularly dust-rich regions) is heated to high temperatures—on the order of a few thousand Kelvin—dust grains are destroyed, and the gas can become ionized or thermally unstable. Under such conditions, star formation is suppressed because the cool, dense pockets of gas necessary for stellar birth are disrupted.

Dust grains typically sublimate at temperatures above 2,000 K. If our sample galaxies host intense radiation fields (either from short-lived starbursts or an AGN), this could explain why they appear dustier while also showing signs that star formation has ceased. Such observations may indicate ongoing dust destruction or clearing processes.

According to \citet{kajisawa_dust_2015}, if we assume that compact star formation at the center is taking place in ID52153, then over the timescale during which emission lines are produced, dust in the central region provides effective self-shielding, allowing star formation to continue. In contrast, the outer regions (or the galaxy as a whole) may contain less dust, and heating by low-mass stars could inhibit the formation of molecular hydrogen, thereby suppressing star formation.

Although Balmer and \oiii\ lines trace ionized regions, they do not easily distinguish whether those regions are ionized by hot stars, AGN radiation, or shocks. More detailed line diagnostics (e.g., BPT diagrams with higher S/N ratios) would help identify the dominant heating mechanism. ALMA observations of the dust continuum can provide constraints on dust temperature and mass. If dust is efficiently destroyed, one might see lower dust masses than expected for the galaxy’s stellar mass or metallicity.





%(Check Draine 2011 textbook).

% heating dust by CMB is not negligible at z>4 (Elisabete da Cunha+13 fig1)
%CMB temperature at z=6.34 Riechers+22 16-30 K
%Grieco+23 Enhanced star formation through the high-temperature formation of H2 on carbonaceous dust grains

\subsubsection{Gas consumption}
A third scenario involves rapid gas consumption through intense, short-lived bursts of star formation. In this ``starburst and fade" picture, a galaxy forms stars at a very high rate for a relatively brief period, quickly using up much of its available cold gas. Another scenario involves a centrally concentrated inflow. Inflows in galaxies refer to the movement of gas toward the galactic center, resulting in mass accumulation that drives star formation and the activity of supermassive black holes. This scenario is also consistent with the observed color differences in this galaxy.
Once the gas supply drops below a critical threshold, star formation effectively shuts down, leading to quenching.


Observations of dusty star-forming galaxies, especially at high redshifts, show that they often experience extremely high star formation rates. If our sample galaxies had a similar starburst phase, the residual warm dust and strong emission lines we see could be the fading traces of that epoch.
In the emission-line regions, the presence of Balmer emission lines indicates relatively recent star formation. However, if the starburst was abrupt and consumed most of the gas, the star-forming regions would decline rapidly afterward, matching the ``early-quenching" nature we observe now. Once again, ALMA or other submillimeter facilities are vital for measuring molecular gas reservoirs. If these galaxies currently have low gas fractions, it would support the rapid gas consumption scenario. High-resolution multi-wavelength IFU can distinguish regions of younger and older stellar populations, offering clues about past starburst activity. If younger stars are confined to small, intense pockets, this would strengthen the ``bursty star-formation then fade" explanation.





\subsubsection{Environmental effects}

In the context of quenching, environmental effects are also significant for low-$z$ cluster galaxies. \citet{morishita_accelerated_2024} reported the discovery of an overdensity at $z\sim5.7$. Among the galaxies in our sample, ID53079 ($z=5.78$) and ID58043 ($z=5.67$) have been identified as members of this protocluster. Because they reside in an overdense region, one possible scenario is that they experienced an elevated merger rate and underwent a burst of star formation, which then ceased. In contrast, ID52153 ($z=5.54$) and ID85007 ($z=5.10$) do not appear to be part of the emitter overdensity, suggesting that environmental effects likely played only a minimal role in their evolution.


